RGA-Net: A Vision Enhancement Framework for Robotic Surgical Systems Using Reciprocal Attention Mechanisms

Robotic surgical systems rely heavily on high-quality visual feedback for precise teleoperation; yet, surgical smoke from energy-based devices significantly degrades endoscopic video feeds, compromising the human-robot interface and surgical outcomes. This paper presents RGA-Net (Reciprocal Gating and Attention-fusion Network), a novel deep learning framework specifically designed for smoke removal in robotic surgery workflows. Our approach addresses the unique challenges of surgical smoke-including dense, non-homogeneous distribution and complex light scattering-through a hierarchical encoder-decoder architecture featuring two key innovations: (1) a Dual-Stream Hybrid Attention (DHA) module that combines shifted window attention with frequency-domain processing to capture both local surgical details and global illumination changes, and (2) an Axis-Decomposed Attention (ADA) module that efficiently processes multi-scale features through factorized attention mechanisms. These components are connected via reciprocal cross-gating blocks that enable bidirectional feature modulation between encoder and decoder pathways. Extensive experiments on the DesmokeData and LSD3K surgical datasets demonstrate that RGA-Net achieves superior performance in restoring visual clarity suitable for robotic surgery integration. Our method enhances the surgeon-robot interface by providing consistently clear visualization, laying a technical foundation for alleviating surgeons' cognitive burden, optimizing operation workflows, and reducing iatrogenic injury risks in minimally invasive procedures. These practical benefits could be further validated through future clinical trials involving surgeon usability assessments. The proposed framework represents a significant step toward more reliable and safer robotic surgical systems through computational vision enhancement.

==> alg.tex <==
\begin{algorithm*}
\caption{RGA-Net Forward Pass}
\label{alg:rganet}
\begin{algorithmic}[1]
\State \textbf{Input:} Input Image $I_{in}$
\State \textbf{Output:} Desmoked Image $I_{out}$

\Function{RGANet}{$I_{in}$}
    \State $X \gets \text{PatchEmbed}(I_{in})$ \Comment{Initial convolution}

    \Comment{--- Encoder Path ---}
    \State $E_1 \gets \text{EncoderLevel1}(X)$ \Comment{Sequence of DHA blocks}
    \State $D_1 \gets \text{Downsample}(E_1)$
    \State $E_2 \gets \text{EncoderLevel2}(D_1)$ \Comment{Sequence of DHA blocks}
    \State $D_2 \gets \text{Downsample}(E_2)$
    \State $E_3 \gets \text{EncoderLevel3}(D_2)$ \Comment{Sequence of DHA blocks}
    \State $D_3 \gets \text{Downsample}(E_3)$

    \Comment{--- Latent Bottleneck ---}
    \State $L \gets \text{Latent}(D_3)$ \Comment{Sequence of ADA blocks}

    \Comment{--- Decoder Path with Reciprocal Gating ---}
    \State $U_3 \gets \text{Upsample}(L)$
    \State $E_{3\_gated}, U_{3\_gated} \gets \text{CrossGating3}(E_3, L)$
    \State $C_3 \gets \text{Concat}(E_{3\_gated}, U_{3\_gated})$
    \State $F_3 \gets \text{ReduceChannels}(C_3)$
    \State $D_3 \gets \text{DecoderLevel3}(F_3)$ \Comment{Sequence of ADA blocks}

    \State $U_2 \gets \text{Upsample}(D_3)$
    \State $E_{2\_gated}, U_{2\_gated} \gets \text{CrossGating2}(E_2, D_3)$
    \State $C_2 \gets \text{Concat}(E_{2\_gated}, U_{2\_gated})$
    \State $F_2 \gets \text{ReduceChannels}(C_2)$
    \State $D_2 \gets \text{DecoderLevel2}(F_2)$ \Comment{Sequence of ADA blocks}

    \State $U_1 \gets \text{Upsample}(D_2)$
    \State $E_{1\_gated}, U_{1\_gated} \gets \text{CrossGating1}(E_1, D_2)$
    \State $C_1 \gets \text{Concat}(E_{1\_gated}, U_{1\_gated})$
    \State $D_1 \gets \text{DecoderLevel1}(C_1)$ \Comment{Sequence of ADA blocks}

    \Comment{--- Refinement and Output ---}
    \State $R \gets \text{Refinement}(D_1)$ \Comment{Sequence of ADA blocks}
    \State $I_{out} \gets \text{OutputConv}(R) + I_{in}$ \Comment{Final convolution and global residual}

    \State \textbf{return} $I_{out}$
\EndFunction
\end{algorithmic}
\end{algorithm*}
